Verifying Exact Samplers for Continuous Distributions with a Discrete Program Logic

Most implementations of sampling algorithms for continuous distributions use floating-point numbers, which introduce round-off errors and approximations. These errors can be difficult to analyze, and can cause security issues when used in algorithms for differential privacy. An alternative is to use exact sampling algorithms based on computable reals, which can lazily generate the digits of a continuous sample to arbitrary precision. However, these algorithms are intricate, and implementing and using them involves a combination of semantically challenging language features, such as probabilistic choice, higher-order functions, and dynamically-allocated mutable state. In this paper we present Continuous-Eris, a higher-order separation logic for verifying the correctness of exact sampling algorithms for computable distributions. To demonstrate Continuous-Eris, we verify the correctness of computable samplers for the uniform, Gaussian, and Laplace distributions, as well as a library for exact real arithmetic for working with generated samples. All of the results in this paper have been verified in the Rocq proof assistant.

==> authors-overrides.tex <==
% Manual overrides for author-name macros.
% Loaded after authors.tex; entries here win.
% Use this for organizational authors, ambiguous "von" forms, etc.

\expandafter\def\csname authname:rocq\endcsname{the Rocq Development Team}
\expandafter\def\csname authname:MPFR\endcsname{the MPFR project}


==> authors.tex <==
% Generated by gen_authors.py from refs.bib -- do not edit by hand.
% Provides \csname authname:KEY\endcsname for each entry; 
% use \authname{key} or \citeauth{key} (see preamble.sty).
\expandafter\def\csname authname:AckermanFR19\endcsname{Ackerman \etal}
\expandafter\def\csname authname:BatzKRW25\endcsname{Batz \etal}
\expandafter\def\csname authname:BeutnerOZ22\endcsname{Beutner \etal}
\expandafter\def\csname authname:DBLP:conf/cca/Muller00\endcsname{M{\"{u}}ller}
\expandafter\def\csname authname:DBLP:conf/csl/BilokonE14\endcsname{Bilokon and Edalat}
\expandafter\def\csname authname:DBLP:conf/esop/HuangM16\endcsname{Huang and Morrisett}
\expandafter\def\csname authname:DBLP:conf/icfp/BorgstromLGS16\endcsname{Borgstr{\"{o}}m \etal}
\expandafter\def\csname authname:DBLP:conf/lics/HeunenKSY17\endcsname{Heunen \etal}
\expandafter\def\csname authname:DBLP:conf/lics/HuotLMS23\endcsname{Huot \etal}
\expandafter\def\csname authname:DBLP:conf/lics/PottsEE97\endcsname{Potts \etal}
\expandafter\def\csname authname:DBLP:conf/mfcs/Simpson98\endcsname{Simpson}
\expandafter\def\csname authname:DBLP:conf/pldi/Boehm20\endcsname{Boehm}
\expandafter\def\csname authname:DBLP:conf/pldi/LeeB90\endcsname{Lee and Boehm}
\expandafter\def\csname authname:DBLP:journals/entcs/BauerK08\endcsname{Bauer and Kavkler}
\expandafter\def\csname authname:DBLP:journals/iandc/Edalat09\endcsname{Edalat}
\expandafter\def\csname authname:DBLP:journals/iandc/Gianantonio96\endcsname{Gianantonio}
\expandafter\def\csname authname:DBLP:journals/pacmpl/Bagnall0023\endcsname{Bagnall \etal}
\expandafter\def\csname authname:DBLP:journals/pacmpl/DahlqvistK20\endcsname{Dahlqvist and Kozen}
\expandafter\def\csname authname:DBLP:journals/pacmpl/EhrhardPT18\endcsname{Ehrhard \etal}
\expandafter\def\csname authname:DBLP:journals/pacmpl/HaselwarterLAGTB25\endcsname{Haselwarter \etal}
\expandafter\def\csname authname:DBLP:journals/pacmpl/HaselwarterLMG024\endcsname{Haselwarter \etal}
\expandafter\def\csname authname:DBLP:journals/pacmpl/VakarKS19\endcsname{V{\'{a}}k{\'{a}}r \etal}
\expandafter\def\csname authname:DBLP:journals/pacmpl/WandCGC18\endcsname{Wand \etal}
\expandafter\def\csname authname:DBLP:journals/tc/Vuillemin90\endcsname{Vuillemin}
\expandafter\def\csname authname:DBLP:journals/tcs/Escardo96\endcsname{Escard{\'{o}}}
\expandafter\def\csname authname:FreerR12\endcsname{Freer and Roy}
\expandafter\def\csname authname:GargHBM24\endcsname{Garg \etal}
\expandafter\def\csname authname:HOYRUP2009830\endcsname{Hoyrup and Rojas}
\expandafter\def\csname authname:HirataMS22\endcsname{Hirata \etal}
\expandafter\def\csname authname:MPFR\endcsname{MPFR}
\expandafter\def\csname authname:Sato16\endcsname{Sato}
\expandafter\def\csname authname:SatoABGGH19\endcsname{Sato \etal}
\expandafter\def\csname authname:Wiedmer1980\endcsname{Wiedmer}
\expandafter\def\csname authname:artifact\endcsname{de Medeiros \etal}
\expandafter\def\csname authname:basl\endcsname{Ho \etal}
\expandafter\def\csname authname:billingsley1995\endcsname{Billingsley}
\expandafter\def\csname authname:clutch\endcsname{Gregersen \etal}
\expandafter\def\csname authname:coneris\endcsname{Li \etal}
\expandafter\def\csname authname:coquelicot\endcsname{Boldo \etal}
\expandafter\def\csname authname:creal\endcsname{Filli{\^{a}}tre}
\expandafter\def\csname authname:dash:lazy\endcsname{Dash \etal}
\expandafter\def\csname authname:dwork14\endcsname{Dwork and Roth}
\expandafter\def\csname authname:eris\endcsname{Aguirre \etal}
\expandafter\def\csname authname:fernandes21\endcsname{Fernandes \etal}
\expandafter\def\csname authname:fullversion\endcsname{de Medeiros \etal}
\expandafter\def\csname authname:ghosh09\endcsname{Ghosh \etal}
\expandafter\def\csname authname:giry\endcsname{Giry}
\expandafter\def\csname authname:huber2016perfect\endcsname{Huber}
\expandafter\def\csname authname:irisjournal\endcsname{Jung \etal}
\expandafter\def\csname authname:karney16\endcsname{Karney}
\expandafter\def\csname authname:lilac\endcsname{Li \etal}
\expandafter\def\csname authname:marionneau:samplers\endcsname{Marionneau \etal}
\expandafter\def\csname authname:menissiermorain:hal-02545650\endcsname{M{\'e}nissier-Morain}
\expandafter\def\csname authname:mevel19\endcsname{M{\'e}vel \etal}
\expandafter\def\csname authname:mironov12\endcsname{Mironov}
\expandafter\def\csname authname:mironov2012significance\endcsname{Mironov}
\expandafter\def\csname authname:occil\endcsname{Occil}
\expandafter\def\csname authname:rocq\endcsname{Team}
\expandafter\def\csname authname:sampcert\endcsname{de Medeiros \etal}
\expandafter\def\csname authname:ub\endcsname{Barthe \etal}
\expandafter\def\csname authname:vonneumann51\endcsname{von Neumann}
\expandafter\def\csname authname:vonneumann63\endcsname{Von Neumann \etal}

